ViQAgent: Zero-Shot Video Question Answering via Agent with Open-Vocabulary Grounding Validation

Recent advancements in Video Question Answering (VideoQA) have introduced LLM-based agents, modular frameworks, and procedural solutions, yielding promising results. These systems use dynamic agents and memory-based mechanisms to break down complex tasks and refine answers. However, significant improvements remain in tracking objects for grounding over time and decision-making based on reasoning to better align object references with language model outputs, as newer models get better at both tasks. This work presents an LLM-brained agent for zero-shot Video Question Answering (VideoQA) that combines a Chain-of-Thought framework with grounding reasoning alongside YOLO-World to enhance object tracking and alignment. This approach establishes a new state-of-the-art in VideoQA and Video Understanding, showing enhanced performance on NExT-QA, iVQA, and ActivityNet-QA benchmarks. Our framework also enables cross-checking of grounding timeframes, improving accuracy and providing valuable support for verification and increased output reliability across multiple video domains. The code is available at https://github.com/t-montes/viqagent.

==> _constants.tex <==
\def\paperID{18656}
\def\confName{CVPR}
\def\confYear{2025}

\def\paperTitle{ViQAgent: Zero-Shot Video Question Answering \\via Agent with Open-Vocabulary Grounding Validation}

\def\authorBlock{
    \textbf{Tony Montes \quad
    Fernando Lozano} \\ 
    The Department of Electrical and Electronics Engineering\\ Universidad de los Andes\\
    {\small \texttt{\{t.montes, flozano\}@uniandes.edu.co}}
}

% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}
